Mass Modelling with Minimum Kinematic Information

Mass modelling of early-type systems is a thorny issue. In this paper, we present a new mass modelling formalism for ellipticals that invokes no observations other than the central velocity dispersion ($\sigma_0$) and photometry. The essence of the method lies in choosing a local mass-to-light ratio ($M/L$) profile for a galaxy, with which the deprojected luminosity density distribution (along the major axis coordinate $x$) is scaled. The resulting discontinuous mass density profile is then smoothed, according to a laid out prescription; the local $M/L$ profile that stems from this smoothed mass density, is found to be significantly different from the raw $M/L$ distribution. A suite of model galaxies (both Sersic and cored in nature) is used for extensive experimentation in order to characterise this raw $M/L$ profile and in each case, the mass density recovered from this mass modelling technique is compared to the known mass distribution. We opt to work with a raw $M/L$ profile that is a simple two-stepped function of $x$, with a low inner and higher outer value of $M/L-\Upsilon_{in}$ and $\Upsilon_{out}$, respectively. The only constraint that we have on this profile is in the centre of the galaxy, via $\sigma_0$. This value of $\sigma_0$ is implemented in the virial theorem to obtain an estimate of the central $M/L$ ratio of the galaxy. The fallibility of the virial mass estimate is taken care of, by allowing for a range in the values of $\Upsilon_{in}$ that can be used for a given galaxy model. Moreover, our experiments indicate that $\Upsilon_{out}$ is uniquely known, for a given $\Upsilon_{in}$; for cored galaxies, this functional form is found uniquely dependant on the core radius. The jump radius of the raw $M/L$ profile is chosen to be thrice the effective radius of the galaxy.

==> dc2 <==
@string{anrev ="An. Revs."}
@string{apj="ApJ"}
@string{apjs="ApJS"}
@string{apjl="ApJLett."}
@string{aj="AJ"}
@string{mnras="MNRAS"}
@string{nature="Nat"}
@string{araa="Ann. Rev. Astron. Astrophys."}
@string{aa="A\&A"}
@string{newast="New Astronomy"}



@article{zepf00,
	author="Zepf, S. E. and Beasley, M. A. and Bridges, T. J. and  Hanes, D. A.and  Sharples, R. M. and  Ashman, K. M. and Geisler, D.",
	title="",
	journal=aj,
	year=2000,
	volume=120,
	pages=2928	}

@article{king66,
	author="King, I. R.",
	title="",
	journal=aj,
	year=1966,
	volume=71,
	pages=64	}

@article{rood72,
	author="Rood, H. J. and Page, T. L. and Kintner, E. C. and King, I. R",
	title="",
	journal=apj,
	year=1972,
	volume=179,
	pages=627	}


@article{hoekstra04,
	author="Hoekstra, H. and Yee, H. K. C. and Gladders, M. D. ",
	title="",
	journal=apj,
	year=2004,
	volume=606,
	pages=67	}


@article{lintott06,
	author="Lintott, C. J. and Ferreras, I. and Lahav, O.",
	title="",
	journal=apj,
	year=2006,
	volume=648,
	pages=826	}

@article{padmanabhan04,
	author="Padmanabhan, N. and Seljak, U. and Strauss, M. A. and Blanton, M. R. and Kauffmann, G. and Schlegel, D. J. and Tremonti, C. and Bahcall, N. A.and Bernardi, M. and Brinkmann, J. and Fukugita, M. and Ivezić, Ž.",
	title="",
	journal=newast,
	year=2004,
	volume=9,
	pages=329	}

@article{verheijen01,
	author="Verheijen, M. A. W.",
	title="",
	journal=apj,
	year=2001,
	volume=563,
	pages=694	}


@article{noordermeer06,
	author="Noordermer, E.",
	title="",
	journal=apj,
	year=2006,
	volume="",
	pages="in preparation"	}

@article{buote,
	author="Buote, D. A. and Jeltema, T. E. and Canizares, C. R. and Garmire, G. P. ",
	title="",
	journal=apj, 
	year=2002,
	volume=577,
	pages=183	}

@article{vdm94,
	author="van der Marel, R. P.",
	title="",
	journal=mnras, 
	year=1994,
	volume=270,
	pages=271	}

@inproceedings{sancisi04,
        author="Sancisi, R.",
        title="",
        booktitle="International Astronomical Union Symposium no. 220",
        editor="Ryder, S. D. and Pisano, D. J. and Walker, M. A. and Freeman, K.",
        year="2004",
        publisher="ASP, San Francisco",
        pages="233",
        notes=""        }

@article{bertola,
	author="Bertola, F. and Pizzella, A. and Persic, M. and Salucci, P.",
	title="",
	journal=apj, 
	year=1993,
	volume=416,
	pages="45L"	}

@article{gebhardt00,
	author="Gebhardt, K. and Bender, R. and Bower, G. and Dressler, A. and Faber, S. M. and Filippenko, A. V. and Green, R. and Grillmair, C. and Ho, L. C. and Kormendy, J. and 5 coauthors",
	title="",
	journal=apj, 
	year=2000,
	volume=539,
	pages="13L"	}

@article{strom81,
        author="Strom, S. E. and Strom, K. M. and Wells, D. C. and Forte, J. C. and Smith, M. G. and Harris, W. E.",
        title="",
        journal=apj,
        year=1981,
        volume=245,
        pages=416       }

@article{dolfdal,
	author="Michielsen, D. and Chakrabarty, D.",
	title="",
	journal=mnras, 
	year=2006,
	volume="",
	pages="in preparation",
        notes=""	}

@article{machetto,
	author="Macchetto, F. and Marconi, A. and Axon, D. J. and Capetti, A. and Sparks, W. and Crane, P.",
	title="",
	journal=apj, 
	year=1997,
	volume=489,
	pages=579	}

@article{napolitano05,
	author="Napolitano, N. R. and Capaccioli, M. and Romanowsky, A. J. and Douglas, N. G. and Merrifield, M. R. and Kuijken, K. and Arnaboldi, M. and Gerhard, O. and Freeman, K. C",
	title="",
	journal=mnras, 
	year=2005,
	volume=357,
	pages=691	}

@book{bible,
      author="Binney, J. and Tremaine, S.",
	title="Galactic Dynamics",
	year=1987,
	publisher="Princeton University Press Princeton New Jersey"	}

@article{gerhardgenzel,
	author="Genzel, R. and Pichon, C. and Eckart, A. and Gerhard, O. E. and Ott, T.",
	title="",
	journal=mnras,
	year=2000,
	volume="317",
	pages="348",
        notes=""	}

@article{doping06,
	author="Chakrabarty, D. and Ferrarese, L.",
	title="",
	journal=aj,
	year="2006",
	volume="",
	pages="submitted to AJ",
        notes=""	}

@article{laura06,
	author="Ferrarese, L. and C\^ot\'e, P. and Jordan, A. and Peng, E. W. and Blakeslee, J. P. and Slawomir P. and Mei, S. and Merritt, D. and Milosavljević, M. and  Tonry, J. L. and West, M. J.",
	title="",
	journal=apjs,
	year=2006,
	volume="164",
	pages="334",
        notes=""	}

@article{cote03,
        author="C\^ot\'e, P. and McLaughlin, D. E. and Cohen, J. G. and Blakeslee, J. P.",
        title="",
        journal=apj,
        year=2003,
        volume=591,
        pages=850}

@article{cote87,
        author="C\^ot\'e, P. and McLaughlin, D.E. and Hanes, D.A. and Bridges, T.J. and Geisl\
er, D. and Merritt, D. and Hesser, J.E. and Harris, G.L.H. and Lee, M.G.",
        title="",
        journal=apj,
        year=2001,
        volume=559,
        pages="828"}

@article{mclaughlin99,
        author="McLaughlin, D.E.",
        title="",
        journal=apj,
        year=1999,
        volume=512,
        pages="L9"}

@article{romkoch87,
        author="Romanowsky, A. J. and Kochanek, C. S.",
        title="",
        journal=apj,
        year=2001,
        volume=553,
        pages="722"}

@article{mamon05,
        author="Mamon, G. A. and {\L}okas, E. L.",
        title="",
        journal=mnras,
        year=2005,
        volume=362,
        pages="95"}

@article{pnsscience,
        author="Romanowsky, A. J. and Douglas, D. N. and Arnaboldi, M. and Kuijken, K. and Merrifield, M. R. and Napolitano, N. R. and Capaccioli, M. and Freeman, K. C.",
        title="",
        journal="Science",
        year=2003,
        volume=301,
        pages="1696"}


@inproceedings{romanowsky04,
        author="Romanowsky, A. J. and Douglas N. G. and Kuijken, K. and Merrifield, M. R.
 and Arnaboldi, A. and Napolitano, N. R. and Merrett, H and Capaccioli, M.",
        title="",
        booktitle="Dark Matter in Galaxies, Proc. IAU Sumposium 220",
        editor="Ryder, S. and Pisano, D. J. and Walker, M. and Freeman, K.",
        year="2004",
        publisher="ASP, San Francisco",
        pages="165",
        notes=""        }

@article{gerhardkronawitter,
        author="Gerhard, O. and Kronawitter, A. and Saglia, R. P. and Bender, R.",
        title="",
        journal=aj,
        year=2001,
        volume="121",
        pages="1936"    }

@article{dalpras,
        author="Chakrabarty, Dalia and Saha, Prasenjit",
        title="",
        journal=aj,
        year=2001,
        volume="122",
        pages="232"     }

@article{dalzwart,
        author = "Chakrabarty, D. and Portegies Zwart, S.",
        title = "",
        journal = aj,
        year = 2004,
        volume = 128,
        pages = 1046 }

@article{merritt93,
        author="Merritt, D.",
        title="",
        journal=apj,
        year=1993,
        volume="413",
        pages="79"}

@article{merritt96,
        author="Merritt, D.",
        title="",
        journal=aj,
        year=1996,
        volume="112",
        pages="1085"}



